SASV Challenge 2022: A Spoofing Aware Speaker Verification Challenge Evaluation Plan

ASV (automatic speaker verification) systems are intrinsically required to reject both non-target (e.g., voice uttered by different speaker) and spoofed (e.g., synthesised or converted) inputs. However, there is little consideration for how ASV systems themselves should be adapted when they are expected to encounter spoofing attacks, nor when they operate in tandem with CMs (spoofing countermeasures), much less how both systems should be jointly optimised. The goal of the first SASV (spoofing-aware speaker verification) challenge, a special sesscion in ISCA INTERSPEECH 2022, is to promote development of integrated systems that can perform ASV and CM simultaneously.

==> tables/Baseline_results_update.tex <==
\begin{table}[ht]
\label{tab:baseline_results}
\caption{
  The three different EERs (\%) for the SASV 2022 development and evaluation partitions.
  SASV-EER for all baselines are calculated using the entire protocol that includes trials used to measure the SV-EER (target vs.\ non-target) and those used to measure the SPF-EER (target vs.\ spoof).
  Results shown for a conventional ASV system (ECAPA-TDNN) and the two baseline solutions.}
\vspace{2mm}
\centerline{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{lcccccc}
\hline

\multirow{2}{*}{} & \multicolumn{2}{c}{SV-EER}  & \multicolumn{2}{c}{SPF-EER} & \multicolumn{2}{c}{SASV-EER}\\ 
\cline{2-7}
                  & \multicolumn{1}{c}{Dev} & \multicolumn{1}{c}{Eval} &  \multicolumn{1}{c}{Dev} & \multicolumn{1}{c}{Eval}& \multicolumn{1}{c}{Dev} & \multicolumn{1}{c}{Eval}               \\ 
\hline

ECAPA-TDNN & 1.24&0.83 & 19.04&29.32 & 16.21&22.38\\
Baseline1 (score-sum)  &14.89&35.1&6.94&0.50&2.09&19.15\\

Baseline2 (back-end ensemble model) &14.38&16.01&0.01&1.23&5.41&8.75\\
\hline
\end{tabular}}
\end{table}

==> tables/baseline2_eer_breakdown.tex <==
\begin{table}[ht]
\label{tab:baseline2_breakdown}
\caption{
  A breakdown of Baseline2 SPF-EER result on the evaluation protocol for each of the 13 different spoofing attacks of the ASVspoof 2019 LA database.
  Results show for the SASV 2022 evaluation protocol.}
\vspace{2mm}
\centerline{
\begin{tabular}{lc}
\hline
Attack type & EER(\%)\\
\hline\hline
A07 & 1.30\\
A08 & 0.30\\
A09 & 0.00\\
A10 & 3.13\\
A11 & 0.14\\
A12 & 1.88\\
A13 & 0.13\\
A14 & 0.13\\
A15 & 0.88\\
A16 & 0.75\\
A17 & 0.89\\
A18 & 1.88\\
A19 & 0.63\\
\hline
pooled&1.23\\

\hline
\end{tabular}}
\end{table}

==> tables/baseline_results.tex <==
\begin{table}[ht]
\label{tab:baseline_results}
\caption{The three different EERs for the SASV 2022 evaluation partition.  Results shown for a conventional ASV system (ECAPA-TDNN) and the two baseline solutions.
%using pre-trained SV and CM systems. We also report min t-DCF for Baseline2.
\textcolor{red}{Max: The min-tDCF here is calculated using scores from SV (target vs non-target) and from CM (target \& non-target vs spoof). Please note that these are the scores produced by the same combined SV-CM system. @Tomi, can you please confirm that nothing is theoretically wrong here?}
\textcolor{blue}{Hemlata: yes Max I double checked with combined SV-CM system (baseline2) using this SV (target vs non-target) and from CM (target \& non-target vs spoof) new update min-tdcf is 0.99865 and CM EER (target \& non-target vs spoof) is 3.4 \%. The min t-dcf legecy one is 0.42539. \\ \\
In row 3 CM-EER is 1.23 \% using CM(target vs. spoof), min t-DCF legacy one 0.37187  (SV (target vs non-target) and from CM (target vs spoof))
%so I think we need to change to 3.4 \% as Prof. Tomi suggested for CM-EER we need to use (target \& non-target vs spoof
). }}
\vspace{2mm}
\centerline{
\begin{tabular}{lcccc}
\hline
 & SV-EER & CM-EER & SASV-EER & min t-DCF \\
\hline\hline
ECAPA-TDNN & 1.24/0.83 & 19.04/29.32 & 16.21/22.38 & -\\
Baseline1  & \multirow{2}{*}{14.89/35.1} & \multirow{2}{*}{6.94/0.50} & \multirow{2}{*}{2.09/19.15} & \multirow{2}{*}{-} \\
(score-sum) \\
Baseline2 & \multirow{2}{*}{14.38/16.01} & \multirow{2}{*}{0.01/1.23} & \multirow{2}{*}{5.41/8.75} & \multirow{2}{*}{0.3718} \\
(back-end ensemble model) \\
\hline
\end{tabular}}
\end{table}
